Deep Learning in Video Multi-Object Tracking: A Survey

The problem of Multiple Object Tracking (MOT) consists in following the trajectory of different objects in a sequence, usually a video. In recent years, with the rise of Deep Learning, the algorithms that provide a solution to this problem have benefited from the representational power of deep models. This paper provides a comprehensive survey on works that employ Deep Learning models to solve the task of MOT on single-camera videos. Four main steps in MOT algorithms are identified, and an in-depth review of how Deep Learning was employed in each one of these stages is presented. A complete experimental comparison of the presented works on the three MOTChallenge datasets is also provided, identifying a number of similarities among the top-performing methods and presenting some possible future research directions.

==> tables/s1_Detection.tex <==
\begin{tabular}{c>{\centering\arraybackslash}p{0.12\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}c>{\centering\arraybackslash}p{0.08\textwidth}}
\toprule
                    & \bfseries Detection                         & Feature extraction / motion prediction                                                      & Affinity computation                                      & Association / Tracking                                                    & Mode & Source and data                                                                                         \\ \midrule
\cite{bewley2016simple}      & Faster R-CNN                      & Kalman filter                                                                   & IoU                                                              & Hungarian algorithm                                                       & O    & \href{https://github.com/abewley/sort}{Source}                                                               \\
\cite{yu2016poi}             & Modified Faster R-CNN             & Modified GoogLeNet, Kalman filter                                               & Cosine distance + IoU                                            & Hungarian algorithm (online), modified H2T \cite{wen2014multiple} (batch) & O+B  & \href{https://drive.google.com/file/d/0B5ACiy41McAHMjczS2p0dFg3emM/view}{Detections and appearance features} \\
%\cite{wojke2017simple}       & From \cite{yu2016poi}             & Kalman filter, Wide Residual Net                                                & Mahalanobis dist. (mot.) + cosine distance (app.), IoU           & Hungarian algorithm                                                       & O    & \href{https://github.com/nwojke/deep_sort}{Source}                                                           \\
%\cite{mahmoudi2019cnnmtt}    & From \cite{yu2016poi}             & CNN                                                                             & appearance + motion + dynamic affinity                           & Hungarian algorithm                                                       & O    &                                                                                                              \\
%\cite{wan2018online}         & From \cite{yu2016poi}             & Kalman filter or LK optical flow, CNN + motion features                         & IoU, Siamese LSTM                                                & Hungarian algorithm                                                       & B    &                                                                                                              \\
\cite{ran2019robust}         & Faster R-CNN                      & CNN (app.), AlphaPose CNN, pose joints velocities, interaction grid & Pose-based Triple Stream Network (LSTM-based)                    & Custom algorithm                                                          & O    &                                                                                                              \\
\cite{hu2018automatic}       & Faster R-CNN                      & CNN                                                                             & Euclidean distance, cosine distance                              & Multifeature fusion re-tracking algorithm                                 & B    &                                                                                                              \\
\cite{zhang2019automatic}    & CNN                               & HOG + Colour Names                                                              & Variation of Discriminative Correlation Filter                   & Custom algorithm + Hungarian algorithm                                    & O    &                                                                                                              \\
\cite{lu2017online}          & SSD                               & SSD, LSTM                                                                       & Cosine similarity                                                & Hungarian algorithm                                                       & O    &                                                                                                              \\
\cite{kieritz2018joint}      & SSD                               & SSD                                                                             & RNN                                                              & Hungarian algorithm, MLP (track scores)                                   & O    &                                                                                                              \\
\cite{zhao2018multi}         & SSD                               & SSD + Correlation Filter                                                        & IoU + APCE                                                       & Hungarian algorithm                                                       & O    &                                                                                                              \\
\cite{zhou2018online}        & Mask R-CNN / Public detections    & Siamese Mask R-CNN                                                              & App. affinity, mot. consistency, spatial structural potential    & Tensor-based high-order graph matching                                    & O    & Code will be released                                                                                        \\
\cite{kim2018online}         & YOLOv2                            & Tiny Yolo, Particle filter, Random Ferns, KLT                                   & Pairwise overlap ratio, student Random Ferns, Euclidean distance & Greedy bipartite assignment                                               & O    &                                                                                                              \\
\cite{sharma2018beyond}      & RRC or SubCNN                     & Feature-based odometry, Pose Adjustment CNN, stacked-hourglass CNN              & 3D-2D cost + 3D-3D cost + appearance, shape and pose costs       & Hungarian algorithm                                                       & O    & \href{https://github.com/JunaidCS032/MOTBeyondPixels}{Source}                                                \\
\cite{pernici2018memory}     & DPM or Tiny (CNN)                 & DPM or Tiny (CNN)                                                               & Implicit in Reverse Nearest Neighbour                            & Reverse Nearest Neighbour Matching                                        & O    & Code will be released                                                                                        \\
\cite{min2018new}            & ViBe + SVM + CNN                  &                                                                                 & IoU                                                              & Region Matching algorithm                                                 & O    &                                                                                                              \\
\cite{bullinger2017instance} & Multi-task Network Cascades (CNN) & Optical flow                                                                    & Overlap of segmentation instances                                & Hungarian algorithm                                                       & O    &                                                                                                             \\ \bottomrule
\end{tabular}

==> tables/s2_Features.tex <==
\begin{tabular}{c>{\centering\arraybackslash}p{0.12\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}c>{\centering\arraybackslash}p{0.08\textwidth}}
\toprule
                              & Detection                                & \bfseries Feature extr. / mot. pred.                                                       & Affinity / cost computation                                                                                      & Association / Tracking                                                                                                      & Mode & Source and data                                                                                                                                                                                               \\ \midrule
\cite{wang2014learning}       & Dalal-Triggs detector                    & Autoencoders                                                                     & SVM                                                                                                              & Minimum spanning tree                                                                                                       & O    &                                                                                                                                                                                                                                   \\
\cite{kim2015multiple}        & Public                                   & CNN + PCA                                                                        & Multi-Output Regularized Least Squares                                                                           & Variation of Multiple Hypothesis Tracking                                                                                   & O    & \href{http://rehg.org/mht/}{Source}                                                                                                                                                                                               \\
\cite{yu2016poi}              & Modified Faster R-CNN                    & Modified GoogLeNet, Kalman filter                                                & Cosine distance + IoU                                                                                            & Hungarian algorithm (online), modified H2T \cite{wen2014multiple} (batch)                                                   & O+B  & \href{https://drive.google.com/file/d/0B5ACiy41McAHMjczS2p0dFg3emM/view}{Detections and appearance features}                                                                                                                      \\
\cite{chen2017enhancing}      & Public                                   & CNN, Kalman Filter                                                               & Multi-Output Regularized Least Squares + Kalman Filter + detection-scene score                                   & Maximum Weighted Independent Set                                                                                            & B    &                                                                                                                                                                                                                                   \\
\cite{yang2017hybrid}         & Public                                   & R-CNN                                                                            & Observation cost + transition cost + birth-death cost                                                            & Min-cost multi commodity flow problem, solved with Dantzig-Wolfe decomposition                                              & O    &                                                                                                                                                                                                                                   \\
\cite{wang2017robust}         & DoH \cite{qian2014automatically}         & CNN                                                                              & CNN + Kalman filter                                                                                              & Custom algorithm, SVM                                                                                                       & B    &                                                                                                                                                                                                                                   \\
\cite{bewley2016simple}       & Faster R-CNN                             & Kalman filter                                                                    & IoU                                                                                                              & Hungarian algorithm                                                                                                         & O    & \href{https://github.com/abewley/sort}{Source}                                                                                                                                                                                    \\
\cite{wojke2017simple}        & From \cite{yu2016poi}                    & Kalman filter, Wide Residual Net                                                 & Mahalanobis dist. (mot.) + cosine distance (app.), IoU                                                           & Hungarian algorithm                                                                                                         & O    & \href{https://github.com/nwojke/deep_sort}{Source}                                                                                                                                                                                \\
\cite{mahmoudi2019cnnmtt}     & From \cite{yu2016poi}                    & CNN                                                                              & appearance + motion + dynamic affinity                                                                           & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{kim2018multi}           & Public                                   & CNN                                                                              & Bilinear LSTM                                                                                                    & Variant of MHT-DAM \cite{kim2015multiple}                                                                                   & B    &                                                                                                                                                                                                                                   \\
\cite{bae2017confidence}      & Public / SDP+RPN                         & CNN                                                                              & Appearance + motion + shape affinities                                                                           & Hungarian algorithm                                                                                                         & O    & \href{https://cvl.gist.ac.kr/project/cmot.html}{Source}                                                                                                                                                                           \\
\cite{ullah2018deep}          & Public                                   & GoogLeNet CNN                                                                    & App. similarity                                                                                                  & Bayesian inference using \cite{pirsiavash2011globally}                                                                      & B    &                                                                                                                                                                                                                                   \\
\cite{fang2018recurrent}      & Public / Faster R-CNN                                  & GoogLeNet CNN                                                                    & Recurrent Autoregressive Networks (GRU-based)                                                                    & Bipartite graph matching                                                                                                    & O    &                                                                                                                                                                                                                                   \\
\cite{fu2018gm}               & Public                                   & CNN                                                                              & Hybrid Likelihood Function (Discriminative Correlation Filter + Gaussian Mixture Probability Hypothesis Density) & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{wen2019learning}        & Public                                   & CNN                                                                              & app. + HSV histogram + motion similarities                                                                       & Pairwise update algorithm + SSVM                                                                                            & B    & Will be available at \href{https://github.com/longyin880815}{this link}                                                                                                                                                           \\
\cite{pernici2018memory}      & DPM or Tiny (CNN)                        & DMP or Tiny (CNN)                                                                & Implicit in Reverse Nearest Neighbour                                                                            & Reverse Nearest Neighbour Matching                                                                                          & O    & Code will be released                                                                                                                                                                                                             \\
\cite{sheng2018heterogeneous} & Public                                   & GoogLeNet CNN, Optical flow                                                      & Distance between app. features, common superpixels, optical flow predictions                                     & Multiple Hypotheses Tracking                                                                                                & B    &                                                                                                                                                                                                                                   \\
\cite{chen2019recurrent}      & Public                                   & CNN                                                                              & LSTM (app.) + motion affinity                                                                                    & Batch Multi-Hypothesis                                                                                                      & B    &                                                                                                                                                                                                                                   \\
\cite{hu2018automatic}        & Faster R-CNN                             & CNN                                                                              & Euclidean distance, cosine distance                                                                              & Multifeature fusion re-tracking algorithm                                                                                   & B    &                                                                                                                                                                                                                                   \\
\cite{ran2019robust}          & Faster R-CNN                             & CNN (app.), AlphaPose CNN, pose joints velocities, interaction grid              & Pose-based Triple Stream Network (LSTM-based)                                                                    & Custom algorithm                                                                                                            & O    &                                                                                                                                                                                                                                   \\
\cite{tang2017multiple}       & Public / From \cite{yu2016poi}            & DeepCut CNN \cite{pishchulin2016deepcut}, StackNetPose CNN                       & StackNetPose CNN                                                                                                 & Lifted multicut problem, solved as in \cite{keuper2015efficient}                                                            & B    & \href{https://www.mpi-inf.mpg.de/departments/computer-vision-and-multimodal-computing/research/people-detection-pose-estimation-and-tracking/multiple-people-tracking-with-lifted-multicut-and-person-re-identification/}{Source} \\
\cite{kim2016similarity}      & Public                                   & Siamese CNN                                                                      & Euclidean distance (app. feat.) + IoU + box area ratio                                                           & Custom greedy algorithm                                                                                                     & O    &                                                                                                                                                                                                                                   \\
\cite{wang2016joint}          & DPM                                      & Siamese CNN with temporal constraints                                            & Mahalanobis distance (app. feat.)  + motion affinity                                                             & Generalized Linear Assignment solved with Softassign \cite{gold1996softmax}, Dual-threshold strategy \cite{huang2008robust} & B    &                                                                                                                                                                                                                                   \\
\cite{zhang2016tracking}      & HeadHunter \cite{benenson2012pedestrian} & CNN                                                                              & Euclidean distance (app. feat.), temporal and kinematic affinities                                               & Hungarian algorithm, Agglomerative clustering                                                                               & B    & \href{https://github.com/shunzhang876/AdaptiveFeatureLearning}{Source}                                                                                                                                                            \\
\cite{leal2016learning}       & Public                                   & Siamese CNN, contextual features                                                 & Gradient Boosting                                                                                                & Linear programming                                                                                                          & B    &                                                                                                                                                                                                                                   \\
\cite{son2017multi}           & Public                                   & CNN, sequence-specific statistics, optical flow, FC layers                       & FC layer combining app. and mot. distances                                                                       & Minimax label propagation                                                                                                   & B    &                                                                                                                                                                                                                                   \\
\cite{zhou2018online}         & Mask R-CNN / Public detections           & Siamese Mask R-CNN                                                               & App. affinity, mot. consistency, spatial structural potential                                                    & Tensor-based high-order graph matching                                                                                      & O    & Code will be released                                                                                                                                                                                                             \\
\cite{maksai2018eliminating}  & Public                                   & CNN + various app. and non-app. feat.                                            & embedding layer + bidirectional LSTM                                                                             & Variation of Multiple Hypothesis Tracking                                                                                   & B    &                                                                                                                                                                                                                                   \\
\cite{zhu2018online}          & Public                                   & Linear motion model, Spatial Attention Network CNN                               & Temporal Attention Network (bidirectional LSTM)                                                                  & Custom greedy algorithm, ECO (SOT tracker)                                                                                  & O    & \href{https://github.com/jizhu1023/DMAN_MOT}{Source}                                                                                                                                                                  \\
\cite{ma2018trajectory}       & Public                                   & Siamese CNN, LSTM, WRN CNN, Siamese Bi-GRU + CNN                                 & Euclidean dist. (app. feat.), spatial distance, GRU feature matching                                             & Hungarian algorithm, bi-GRU RNN (track split), custom algorithm                                                             & B    &                                                                                                                                                                                                                                   \\
\cite{zhou2018deep}           & Public                                   & DCCRF, visual-displacement CNN                                                   & Visual-similarity CNN, IoU                                                                                       & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{long2018tracking}           & Public                                   & R-FCN + Kalman Filter, GoogleNet                                                 & Eucl. dist. (app. feat.), IoU                                                                                    & Hierarchical Data Association                                                                                               & O    & \href{https://github.com/longcw/MOTDT}{Source}                                                                                                                                                                                                                                  \\
\cite{lee2019multiple}        & Public                                   & Feature Pyramid Siamese Network, motion features                                 & Feature Pyramid Siamese Network                                                                                  & Custom greedy algorithm                                                                                                     & O    &                                                                                                                                                                                                                                   \\
\cite{lu2017online}           & SSD                                      & SSD, LSTM                                                                        & Cosine similarity                                                                                                & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{ullah2017hierarchical}  & Public                    & Kalman Filter, GoogLeNet                                                         & Distance between sparse coding of features using a learned dictionary                  & Hungarian algorithm                                                                                                         & B    &                                                                                                                                                                                                                                   \\
\cite{sadeghian2017tracking}  & Public                                   & 3 LSTMs (app., mot., interaction features) using CNN, bb velocity, occupancy map & LSTM                                                                                                             & Hungarian algorithm, SOT tracker \cite{xiang2015learning}                                                                   & O    &                                                                                                                                                                                                                                   \\
\cite{chu2017online}          & Public                                   & Linear motion model, CNN                                                         & CNN                                                                                                              & Association to highest classification score                                                                                 & O    &                                                                                                                                                                                                                                   \\
\cite{sharma2018beyond}       & RRC or SubCNN                            & Feature-based odometry, Pose Adjustment CNN, stacked-hourglass CNN               & 3D-2D cost + 3D-3D cost + appearance, shape and pose costs                                                       & Hungarian algorithm                                                                                                         & O    & \href{https://github.com/JunaidCS032/MOTBeyondPixels}{Source}                                                                                                                                                                     \\
\cite{kim2018online}          & YOLOv2                                   & Tiny Yolo, Particle filter, Random Ferns, KLT                                    & Pairwise overlap ratio, student Random Ferns, Euclidean distance                                                 & Greedy bipartite assignment                                                                                                 & O    &                                                                                                                                                                                                                                   \\
\cite{ullah2018directed}      & Manually generated                       & Hidden Markov Models, CNN                                                        & Mutual information (app. feat.)                                                                                  & Dynamic programming algorithm from \cite{pirsiavash2011globally}                                                            & B    &                                                                                                                                                                                                                                   \\
\cite{wang2017online}         & Public                                   & LK optical flow, Convolutional Correlation Filter CNN, Kalman filter             & Optical flow aff., app. feat. aff., IoU, scale affinity, distance between detections                             & Custom algorithm (with Hungarian alg.)                                                                                      & O    & \href{http://faculty.neu.edu.cn/ise/wanglu/CCF_MOT.htm}{Source}                                                                                                                                                                   \\
\cite{zhao2018multi}          & SSD                                      & SSD + Correlation Filter                                                         & IoU + APCE                                                                                                       & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{rosello2018multi}       & Public                                   & Kalman filter + Deep RL agent                                                    & IoU                                                                                                              & Hungarian algorithm + Deep RL agent                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{babaee2018occlusion}    & N/A                                      & LSTM (mot.)                                                                      & Stitching score using IoU                                                                                        & Custom iterative tracklet-stitching algorithm                                                                               & B    &                                                                                                                                                                                                                                  \\ \bottomrule
\end{tabular}

==> tables/s2_Features_longtable.tex <==
\begin{longtable}{c>{\centering\arraybackslash}p{0.12\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}c>{\centering\arraybackslash}p{0.08\textwidth}}
\toprule
                              & Detection                                & \bfseries Feature extr. / mot. pred.                                                       & Affinity / cost computation                                                                                      & Association / Tracking                                                                                                      & Mode & Source and data                                                                                                                                                                                               \\ \midrule \endhead
                              \hline
 \endfoot
 \endlastfoot
\cite{wang2014learning}       & Dalal-Triggs detector                    & Autoencoders                                                                     & SVM                                                                                                              & Minimum spanning tree                                                                                                       & O    &                                                                                                                                                                                                                                   \\
\cite{kim2015multiple}        & Public                                   & CNN + PCA                                                                        & Multi-Output Regularized Least Squares                                                                           & Variation of Multiple Hypothesis Tracking                                                                                   & O    & \href{http://rehg.org/mht/}{Source}                                                                                                                                                                                               \\
\cite{yu2016poi}              & Modified Faster R-CNN                    & Modified GoogLeNet, Kalman filter                                                & Cosine distance + IoU                                                                                            & Hungarian algorithm (online), modified H2T \cite{wen2014multiple} (batch)                                                   & O+B  & \href{https://drive.google.com/file/d/0B5ACiy41McAHMjczS2p0dFg3emM/view}{Detections and appearance features}                                                                                                                      \\
\cite{chen2017enhancing}      & Public                                   & CNN, Kalman Filter                                                               & Multi-Output Regularized Least Squares + Kalman Filter + detection-scene score                                   & Maximum Weighted Independent Set                                                                                            & B    &                                                                                                                                                                                                                                   \\
\cite{yang2017hybrid}         & Public                                   & R-CNN                                                                            & Observation cost + transition cost + birth-death cost                                                            & Min-cost multi commodity flow problem, solved with Dantzig-Wolfe decomposition                                              & O    &                                                                                                                                                                                                                                   \\
\cite{wang2017robust}         & DoH \cite{qian2014automatically}         & CNN                                                                              & CNN + Kalman filter                                                                                              & Custom algorithm, SVM                                                                                                       & B    &                                                                                                                                                                                                                                   \\
\cite{bewley2016simple}       & Faster R-CNN                             & Kalman filter                                                                    & IoU                                                                                                              & Hungarian algorithm                                                                                                         & O    & \href{https://github.com/abewley/sort}{Source}                                                                                                                                                                                    \\
\cite{wojke2017simple}        & From \cite{yu2016poi}                    & Kalman filter, Wide Residual Net                                                 & Mahalanobis dist. (mot.) + cosine distance (app.), IoU                                                           & Hungarian algorithm                                                                                                         & O    & \href{https://github.com/nwojke/deep_sort}{Source}                                                                                                                                                                                \\
\cite{mahmoudi2019cnnmtt}     & From \cite{yu2016poi}                    & CNN                                                                              & appearance + motion + dynamic affinity                                                                           & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{kim2018multi}           & Public                                   & CNN                                                                              & Bilinear LSTM                                                                                                    & Variant of MHT-DAM \cite{kim2015multiple}                                                                                   & B    &                                                                                                                                                                                                                                   \\
\cite{bae2017confidence}      & Public / SDP+RPN                         & CNN                                                                              & Appearance + motion + shape affinities                                                                           & Hungarian algorithm                                                                                                         & O    & \href{https://cvl.gist.ac.kr/project/cmot.html}{Source}                                                                                                                                                                           \\
\cite{ullah2018deep}          & Public                                   & GoogLeNet CNN                                                                    & App. similarity                                                                                                  & Bayesian inference using \cite{pirsiavash2011globally}                                                                      & B    &                                                                                                                                                                                                                                   \\
\cite{fang2018recurrent}      & Public / Faster R-CNN                                  & GoogLeNet CNN                                                                    & Recurrent Autoregressive Networks (GRU-based)                                                                    & Bipartite graph matching                                                                                                    & O    &                                                                                                                                                                                                                                   \\
\cite{fu2018gm}               & Public                                   & CNN                                                                              & Hybrid Likelihood Function (Discriminative Correlation Filter + Gaussian Mixture Probability Hypothesis Density) & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{wen2019learning}        & Public                                   & CNN                                                                              & app. + HSV histogram + motion similarities                                                                       & Pairwise update algorithm + SSVM                                                                                            & B    & Will be available at \href{https://github.com/longyin880815}{this link}                                                                                                                                                           \\
\cite{pernici2018memory}      & DPM or Tiny (CNN)                        & DMP or Tiny (CNN)                                                                & Implicit in Reverse Nearest Neighbour                                                                            & Reverse Nearest Neighbour Matching                                                                                          & O    & Code will be released                                                                                                                                                                                                             \\
\cite{sheng2018heterogeneous} & Public                                   & GoogLeNet CNN, Optical flow                                                      & Distance between app. features, common superpixels, optical flow predictions                                     & Multiple Hypotheses Tracking                                                                                                & B    &                                                                                                                                                                                                                                   \\
\cite{chen2019recurrent}      & Public                                   & CNN                                                                              & LSTM (app.) + motion affinity                                                                                    & Batch Multi-Hypothesis                                                                                                      & B    &                                                                                                                                                                                                                                   \\
\cite{hu2018automatic}        & Faster R-CNN                             & CNN                                                                              & Euclidean distance, cosine distance                                                                              & Multifeature fusion re-tracking algorithm                                                                                   & B    &                                                                                                                                                                                                                                   \\
\cite{ran2019robust}          & Faster R-CNN                             & CNN (app.), AlphaPose CNN, pose joints velocities, interaction grid              & Pose-based Triple Stream Network (LSTM-based)                                                                    & Custom algorithm                                                                                                            & O    &                                                                                                                                                                                                                                   \\
\cite{tang2017multiple}       & Public / From \cite{yu2016poi}           & DeepCut CNN \cite{pishchulin2016deepcut}, StackNetPose CNN                       & StackNetPose CNN                                                                                                 & Lifted multicut problem, solved as in \cite{keuper2015efficient}                                                            & B    & \href{https://www.mpi-inf.mpg.de/departments/computer-vision-and-multimodal-computing/research/people-detection-pose-estimation-and-tracking/multiple-people-tracking-with-lifted-multicut-and-person-re-identification/}{Source} \\
\cite{kim2016similarity}      & Public                                   & Siamese CNN                                                                      & Euclidean distance (app. feat.) + IoU + box area ratio                                                           & Custom greedy algorithm                                                                                                     & O    &                                                                                                                                                                                                                                   \\
\cite{wang2016joint}          & DPM                                      & Siamese CNN with temporal constraints                                            & Mahalanobis distance (app. feat.)  + motion affinity                                                             & Generalized Linear Assignment solved with Softassign \cite{gold1996softmax}, Dual-threshold strategy \cite{huang2008robust} & B    &                                                                                                                                                                                                                                   \\
\cite{zhang2016tracking}      & HeadHunter \cite{benenson2012pedestrian} & CNN                                                                              & Euclidean distance (app. feat.), temporal and kinematic affinities                                               & Hungarian algorithm, Agglomerative clustering                                                                               & B    & \href{https://github.com/shunzhang876/AdaptiveFeatureLearning}{Source}                                                                                                                                                            \\
\cite{leal2016learning}       & Public                                   & Siamese CNN, contextual features                                                 & Gradient Boosting                                                                                                & Linear programming                                                                                                          & B    &                                                                                                                                                                                                                                   \\
\cite{son2017multi}           & Public                                   & CNN, sequence-specific statistics, optical flow, FC layers                       & FC layer combining app. and mot. distances                                                                       & Minimax label propagation                                                                                                   & B    &                                                                                                                                                                                                                                   \\
\cite{zhou2018online}         & Mask R-CNN / Public detections           & Siamese Mask R-CNN                                                               & App. affinity, mot. consistency, spatial structural potential                                                    & Tensor-based high-order graph matching                                                                                      & O    & Code will be released                                                                                                                                                                                                             \\
\cite{maksai2018eliminating}  & Public                                   & CNN + various app. and non-app. feat.                                            & embedding layer + bidirectional LSTM                                                                             & Variation of Multiple Hypothesis Tracking                                                                                   & B    &                                                                                                                                                                                                                                   \\
\cite{zhu2018online}          & Public                                   & Linear motion model, Spatial Attention Network CNN                               & Temporal Attention Network (bidirectional LSTM)                                                                  & Custom greedy algorithm, ECO (SOT tracker)                                                                                  & O    & \href{https://github.com/jizhu1023/DMAN_MOT}{Source}                                                                                                                                                                 \\
\cite{ma2018trajectory}       & Public                                   & Siamese CNN, LSTM, WRN CNN, Siamese Bi-GRU + CNN                                 & Euclidean dist. (app. feat.), spatial distance, GRU feature matching                                             & Hungarian algorithm, bi-GRU RNN (track split), custom algorithm                                                             & B    &                                                                                                                                                                                                                                   \\
\cite{zhou2018deep}           & Public                                   & DCCRF, visual-displacement CNN                                                   & Visual-similarity CNN, IoU                                                                                       & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{long2018tracking}           & Public                                   & R-FCN + Kalman Filter, GoogleNet                                                 & Eucl. dist. (app. feat.), IoU                                                                                    & Hierarchical Data Association                                                                                               & O    & \href{https://github.com/longcw/MOTDT}{Source}                                                                                                                                                                                                                                  \\
\cite{lee2019multiple}        & Public                                   & Feature Pyramid Siamese Network, motion features                                 & Feature Pyramid Siamese Network                                                                                  & Custom greedy algorithm                                                                                                     & O    &                                                                                                                                                                                                                                   \\
\cite{lu2017online}           & SSD                                      & SSD, LSTM                                                                        & Cosine similarity                                                                                                & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{ullah2017hierarchical}  & Public                    & Kalman Filter, GoogLeNet                                                         &  Distance between sparse coding of features using a learned dictionary                                                                                                  & Hungarian algorithm                                                                                                         & B    &                                                                                                                                                                                                                                   \\
\cite{sadeghian2017tracking}  & Public                                   & 3 LSTMs (app., mot., interaction features) using CNN, bb velocity, occupancy map & LSTM                                                                                                             & Hungarian algorithm, SOT tracker \cite{xiang2015learning}                                                                   & O    &                                                                                                                                                                                                                                   \\
\cite{chu2017online}          & Public                                   & Linear motion model, CNN                                                         & CNN                                                                                                              & Association to highest classification score                                                                                 & O    &                                                                                                                                                                                                                                   \\
\cite{sharma2018beyond}       & RRC or SubCNN                            & Feature-based odometry, Pose Adjustment CNN, stacked-hourglass CNN               & 3D-2D cost + 3D-3D cost + appearance, shape and pose costs                                                       & Hungarian algorithm                                                                                                         & O    & \href{https://github.com/JunaidCS032/MOTBeyondPixels}{Source}                                                                                                                                                                     \\
\cite{kim2018online}          & YOLOv2                                   & Tiny Yolo, Particle filter, Random Ferns, KLT                                    & Pairwise overlap ratio, student Random Ferns, Euclidean distance                                                 & Greedy bipartite assignment                                                                                                 & O    &                                                                                                                                                                                                                                   \\
\cite{ullah2018directed}      & Manually generated                       & Hidden Markov Models, CNN                                                        & Mutual information (app. feat.)                                                                                  & Dynamic programming algorithm from \cite{pirsiavash2011globally}                                                            & B    &                                                                                                                                                                                                                                   \\
\cite{wang2017online}         & Public                                   & LK optical flow, Convolutional Correlation Filter CNN, Kalman filter             & Optical flow aff., app. feat. aff., IoU, scale affinity, distance between detections                             & Custom algorithm (with Hungarian alg.)                                                                                      & O    & \href{http://faculty.neu.edu.cn/ise/wanglu/CCF_MOT.htm}{Source}                                                                                                                                                                   \\
\cite{zhao2018multi}          & SSD                                      & SSD + Correlation Filter                                                         & IoU + APCE                                                                                                       & Hungarian algorithm                                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{rosello2018multi}       & Public                                   & Kalman filter + Deep RL agent                                                    & IoU                                                                                                              & Hungarian algorithm + Deep RL agent                                                                                         & O    &                                                                                                                                                                                                                                   \\
\cite{babaee2018occlusion}    & N/A                                      & LSTM (mot.)                                                                      & Stitching score using IoU                                                                                        & Custom iterative tracklet-stitching algorithm                                                                               & B    &                                                                                                                                                                                                                                  \\ \bottomrule
\caption{Information summary about methods using DL for feature extraction or motion prediction. \textit{app.} means appearance, \textit{mot.} means motion, \textit{feat.} means features; \textit{O} and \textit{B} in the Mode column indicate Online and Batch methods respectively. Text in the last column is clickable and contains links to the specified data.}\\
\label{tab:summary_feat}\\
\end{longtable}

==> tables/s3_Affinity.tex <==
% Check reference 78, not sure if should be included in the table

\begin{tabular}{c>{\centering\arraybackslash}p{0.12\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}c>{\centering\arraybackslash}p{0.08\textwidth}}
\toprule
                             & Detection                                                          & Feature extr. / mot. pred.                                                       & \bfseries Affinity / cost computation                            & Association / Tracking                                           & Mode & Source and data                                                                                                                                                                                                              \\ \midrule
\cite{milan2017online}       & Public                                                             & RNN (mot.)                                                                       & LSTM                                                   & RNN                                                              & O    & \href{https://bitbucket.org/amilan/rnntracking}{Source}                                                                                                                                                                           \\
\cite{sadeghian2017tracking} & Public                                                             & 3 LSTMs (app., mot., interaction features) using CNN, bb velocity, occupancy map & LSTM                                                   & Hungarian algorithm, SOT tracker \cite{xiang2015learning}        & O    &                                                                                                                                                                                                                                   \\
\cite{ran2019robust}         & Faster R-CNN                                                       & CNN (app.), AlphaPose CNN, pose joints velocities, interaction grid              & Pose-based Triple Stream Network (LSTM-based)          & Custom algorithm                                                 & O    &                                                                                                                                                                                                                                   \\
\cite{liang2018lstm}         & Public                                                             & 2 LSTMs, VGG16 CNN                                                               & SVM, Siamese LSTM                                      & Greedy association                                               & B    &                                                                                                                                                                                                                                   \\
\cite{wan2018online}         & From \cite{yu2016poi}                                              & Kalman filter or LK optical flow, CNN + motion features                          & IoU, Siamese LSTM                                      & Hungarian algorithm                                              & B    &                                                                                                                                                                                                                                   \\
\cite{zhu2018online}         & Public                                                             & Linear motion model, Spatial Attention Network CNN                               & Temporal Attention Network (bidirectional LSTM)        & Custom greedy algorithm, ECO (SOT tracker)                       & O    & \href{https://github.com/jizhu1023/DMAN_MOT}{Source}                                                                                                                                                                       \\
\cite{yoon2019data}          & Public                                                             &                                                                                  & FC layers + Bi-directional LSTM                        & Hungarian algorithm                                              & O    &                                                                                                                                                                                                                                   \\
\cite{kim2018multi}          & Public                                                             & CNN                                                                              & Bilinear LSTM                                          & Variant of MHT-DAM \cite{kim2015multiple}                        & B    &                                                                                                                                                                                                                                   \\
\cite{kim2015multiple}       & Public                                                             & CNN + PCA                                                                        & Multi-Output Regularized Least Squares                 & Variation of Multiple Hypothesis Tracking                        & O    & \href{http://rehg.org/mht/}{Source}                                                                                                                                                                                               \\
\cite{maksai2018eliminating} & Public                                                             & CNN + various app. and non-app. feat.                                            & embedding layer + bidirectional LSTM                   & Variation of Multiple Hypothesis Tracking                        & B    &                                                                                                                                                                                                                                   \\
\cite{chen2019recurrent}     & Public                                                             & CNN                                                                              & LSTM (app.) + motion affinity                          & Batch Multi-Hypothesis                                           & B    &                                                                                                                                                                                                                                   \\
\cite{fang2018recurrent}     & Public / Faster R-CNN                                                             & GoogLeNet CNN                                                                    & Recurrent Autoregressive Networks (GRU-based)          & Bipartite graph matching                                         & O    &                                                                                                                                                                                                                                   \\
\cite{kieritz2018joint}      & SSD                                                                & SSD                                                                              & RNN                                                    & Hungarian algorithm, MLP (track scores)                          & O    &                                                                                                                                                                                                                                   \\
\cite{tang2017multiple}      & Public / From \cite{yu2016poi}                           & DeepCut CNN \cite{pishchulin2016deepcut}, StackNetPose CNN                       & StackNetPose CNN                                       & Lifted multicut problem, solved as in \cite{keuper2015efficient} & B    & \href{https://www.mpi-inf.mpg.de/departments/computer-vision-and-multimodal-computing/research/people-detection-pose-estimation-and-tracking/multiple-people-tracking-with-lifted-multicut-and-person-re-identification/}{Source} \\
\cite{chen2017online}        & Public / from \cite{sanchez2016online} (combines DPM, SDP and ACF) & Modified Faster R-CNN                                                            & Modified Faster R-CNN                                  & Particle filter                                                  & O    &                                                                                                                                                                                                                                   \\
\cite{zhou2018deep}          & Public                                                             & DCCRF, visual-displacement CNN                                                   & Visual-similarity CNN, IoU                             & Hungarian algorithm                                              & O    &                                                                                                                                                                                                                                   \\
\cite{ma2018customized}      & Public                                                             & DeepMatching, Siamese CNN                                                        & Edge potential as in \cite{tang2016multi}, Siamese CNN & Lifted multicut                                                  & B    &                                                                                                                                                                                                                                   \\
\cite{lee2019multiple}       & Public                                                             & Feature Pyramid Siamese Network, motion features                                 & Feature Pyramid Siamese Network                        & Custom greedy algorithm                                          & O    &                                                                                                                                                                                                                                  \\ \bottomrule
\end{tabular}

==> tables/s4_Association.tex <==
\begin{tabular}{c>{\centering\arraybackslash}p{0.12\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}c>{\centering\arraybackslash}p{0.08\textwidth}}
\toprule
                             & Detection                                                          & Feature extr. / mot. pred.                                                       & Affinity / cost computation                            & \bfseries Association / Tracking                                           & Mode & Source and data                                                                                                                                                                                                              \\ \midrule
\cite{milan2017online}      & Public    & RNN (mot.)                                       & LSTM                                                                 & RNN                                                             & O    & \href{https://bitbucket.org/amilan/rnntracking}{Source} \\
\cite{ma2018trajectory}     & Public    & Siamese CNN, LSTM, WRN CNN, Siamese Bi-GRU + CNN & Euclidean dist. (app. feat.), spatial distance, GRU feature matching & Hungarian algorithm, bi-GRU RNN (track split), custom algorithm & B    &                                                         \\
\cite{kieritz2018joint}     & SSD       & SSD                                              & RNN                                                                  & Hungarian algorithm, MLP (track scores)                         & O    &                                                         \\
\cite{rosello2018multi}     & Public    & Kalman filter + Deep RL agent                    & IoU                                                                  & Hungarian algorithm + Deep RL agent                             & O    &                                                         \\
\cite{ren2018collaborative} & Public    & CNN (motion pred.), part of MDNet (CNN)          & N/A                                                                  & Deep RL agents                                                  & O    &                                                        \\ \bottomrule
\end{tabular}
